Stable interpolation with isotropic and anisotropic Gaussians using Hermite generating function

Gaussian kernels can be an efficient and accurate tool for multivariate interpolation. In practice, high accuracies are often achieved in the flat limit where the interpolation matrix becomes increasingly ill-conditioned. Stable evaluation algorithms for isotropic Gaussians (Gaussian radial basis functions) have been proposed based on a Chebyshev expansion of the Gaussians by Fornberg, Larsson & Flyer and based on a Mercer expansion with Hermite polynomials by Fasshauer & McCourt. In this paper, we propose a new stabilization algorithm for the multivariate interpolation with isotropic or anisotropic Gaussians derived from the generating function of the Hermite polynomials. We also derive and analyse a new analytic cut-off criterion for the generating function expansion that allows to automatically adjust the number of the stabilizing basis functions.

==> Sections/stableImplementation.tex <==
\subsection{Stable implementation}\label{sec:implementation}
Even though the described approach allows to reduce the ill-conditioning of the collocation and evaluation matrices, the HermiteGF-based matrices still become increasingly ill-conditioned for growing number of basis functions. On the other hand, the product of the evaluation matrix $\Psi(X^{\mathrm{eval}})$ and the inverse of the collocation matrix $\Psi(X^{\mathrm{col}})$ is still well-conditioned. For this reason, it is crucial to take special care when building these matrices and inverting the collocation matrix.
The following configurations have proven to be preferable:
\begin{itemize}
 \item First compute $\Psi(X_{\ell}^{\mathrm{eval}})\Psi(X_{\ell}^{\mathrm{col}})^{-1}$  which allows to reduce ill-conditioning.\\
 Using the built-in operator \texttt{/} for the inversion yields good results in \texttt{MATLAB}. 
 \item The HermiteGF basis functions can be stabely evaluated by formulating them in terms of the $d$-dimensional tensor product Hermite functions $\psi_{\lbb}$,
\begin{equation*}
\haggf(\bx) =  \pi^{d/4}t^{\vert \lbb \vert/2}\psi_{\lbb}(G^T x)\exp\left(\bx^T\left(E^TE - \frac{1}{2}GG^T\right)\bx\right).
\end{equation*}
Hermite functions can be stabely evaluated based on their three-term recurrence. 
\end{itemize}

